Prompt to Polyp: Medical Text-Conditioned Image Synthesis with Diffusion Models

The generation of realistic medical images from text descriptions has significant potential to address data scarcity challenges in healthcare AI while preserving patient privacy. This paper presents a comprehensive study of text-to-image synthesis in the medical domain, comparing two distinct approaches: (1) fine-tuning large pre-trained latent diffusion models and (2) training small, domain-specific models. We introduce a novel model named MSDM, an optimized architecture based on Stable Diffusion that integrates a clinical text encoder, variational autoencoder, and cross-attention mechanisms to better align medical text prompts with generated images. Our study compares two approaches: fine-tuning large pre-trained models (FLUX, Kandinsky) versus training compact domain-specific models (MSDM). Evaluation across colonoscopy (MedVQA-GI) and radiology (ROCOv2) datasets reveals that while large models achieve higher fidelity, our optimized MSDM delivers comparable quality with lower computational costs. Quantitative metrics and qualitative evaluations by medical experts reveal strengths and limitations of each approach.

==> models.tex <==
\section{Models}
Most teams utilized COVID-related BERT models for \task{}, along with additional techniques like regularized dropout (R-drop), to address issues with unbalanced label distribution and overfitting; see \cite{weissenbacher-etal-2022-overview} for F1 scores for each of the 14 team’s best-performing system for both tasks.

In this paper, we focus on three key model characteristics: (i) aggregation of claim and tweet texts as input data of a language model, (ii) syntactic features, and (iii) dual-view architecture that learns the representations of both types of texts.
In this regard, we employed models that proved their robustness for stance and premise detection in tweets related to COVID-19 and were ranked as the top-5 best-performing architectures during \task{}: BART + syntax features \cite{das-etal-2022-enolp} and DAN-Bert \cite{yang-etal-2022-yiriyou}. Each model leveraged different techniques to capture the nuanced information in the tweets. All the used models were trained in two set-ups: basic (utilizing the tweets only) and with the adoption of the early fusion technique \cite{early-fusion}. Early fusion employs concatenated features from two modalities (tweets texts and corresponding claims) as input features for the classifiers. The models used in our research are described below.


\subsection{BERT-base model}
Since Transformer-based models \cite{NIPS2017_3f5ee243} produce robust context-based representations of textual data, we leverage BERT-base-uncased as our base model to solve the premise and stance detection task. 
This is a BERT model consisting of 12 layers of Transformer encoder, 12 attention heads, 768 hidden size, and 110M parameters \cite{devlin2018pretraining}; we fine-tuned the model for the text classification tasks on our data. 

\subsection{BART + Syntax features} 

One of the best-performing models in \task{} leveraged the syntactic features of the text. Thus, we included this model in the comparison. This model is based on BART architecture \cite{lewis-etal-2020-bart}, an encoder-decoder transformer model with a BERT-like bidirectional encoder and auto-regressive decoder like GPT. Since BART's pre-training task encourages the model to learn representations that are robust to noise and variations in the input text, the model is well-suited for tasks that require handling noisy and ambiguous text.
To capture the syntactic structure of the input sentences, we incorporate a feature obtained from the dependency parse tree of the sentence. We leverage the open-source tool Spacy \cite{spacy2} to construct the dependency parse tree. Following that, the dependency features are encoded in descending order of their occurrence. Consider three distinct dependency tags: `aux', `amod', `nsubj' in all of the input sentences in the original dataset. If `aux', `nsubj', and `amod' have their occurrence count in the order mentioned, then `aux', `nsubj', and `amod' are encoded as one, two, and three, respectively. These encoded features are concatenated to the transformer model's output and fed into the classifier head to obtain the stance/premise. 
Instead of the usual cross-entropy loss, the supervised contrastive
loss function \cite{NEURIPS2020_d89a66c7} was used. This helped leverage label information better and morph the embedding space by pulling data points from the same class closer and pushing apart data points from other classes.
The dataset for contrastive training was created
by adding positive and negative labels to the samples present in the task dataset. We try three different strategies: fine-tuning with contrastive loss only, pre-training with contrastive loss, then fine-tuning with cross-entropy loss, and fine-tuning with a weighted loss with 0.7 weight given to cross-entropy and 0.3 to contrastive loss. The weights
were chosen considering the performance when
fine-tuning with cross-entropy and contrastive loss.

\subsection{COVID-Twitter-BERT}
BERT-large-uncased model, pre-trained on 97M unique tweets (1.2B training examples) collected between January 12 and July 5, 2020, containing at least one of the keywords ``wuhan'', ``ncov'', ``coronavirus'', ``covid'', or ``sars-cov-2''. These tweets were filtered and preprocessed to reach a final sample of 22.5M tweets (containing 40.7M sentences and 633M tokens), which were used for training \cite{muller2020covid}. We fine-tuned this model for our two classification tasks: binary classification for Premise detection and 3-class classification for Stance prediction. 
The following parameters were leveraged during this fine-tuning. Cross-entropy was leveraged as a loss function with the learning rate set to 4,00E-05. We also used AdamW \cite{loshchilov2018decoupled} as an optimizer with the weight decay set to 0. We trained the model for $10$ epochs with the batch size set to $8$ and the maximum sequence length set to 128. 

\subsection{DAN-BERT}
This architecture draws inspiration from the dual-view adaptation neural network \citep{xu2020dan}, which learns both representations of subjective and objective features of texts. Fig. \ref{fig:model} presents the overall system architecture. 

Given a tokenized tweet, the output embedding of [CLS] token is obtained through the COVID-Twitter-BERT-v2 model \cite{muller2020covid}, which is a pre-trained BERT model on a large corpus of tweets regarding COVID-19 and is the latest version with better downstream performance \footnote{\url{https://huggingface.co/digitalepidemiologylab/covid-twitter-bert-v2}}.  [CLS] is a special classification token and the last hidden state of BERT which is used for classification tasks. We employ it because of its ability to capture a representation of the whole sequence. 

\begin{figure}[t!]
    \centering
    \includegraphics[scale=0.31]{graphs/System.eps}
    \caption{The overall dual-view architecture. The text is tokenized with a [CLS] token and a [SEP] token added at the beginning and end, respectively. The tokens are passed through the pre-trained language models to get their corresponding embeddings, followed by a fusion block and a classifier.}
    \label{fig:model}
\end{figure}

For extracting subjective and objective information separately, the [CLS] token is duplicated and passed through two COVID-Twitter-BERT-v2 models to obtain the corresponding embeddings (i.e., subjective and objective feature vectors, denoted by $\bm{f}_{subj}$ and $\bm{f}_{obj}$, respectively).

These two embeddings are then concatenated and fed into a fusion block composed of a fully connected layer with hidden dimensions of 2048 and a sigmoid activation function to produce a weight vector as follows,


\begin{equation}
\label{eq1}
\bm{\alpha} = {\rm sigmoid} (\bm{W}[\bm{f}_{subj}, \bm{f}_{obj}] + \bm{b}),  
\end{equation} 
where $\left[,\right]$ denotes vector concatenation and $\bm{W}, \bm{b} $ are trainable parameters. 
\par
The goal of the fusion block is to attain an optimal combination between $\bm{f}_{subj}$ and $\bm{f}_{obj}$. Once the weight vector $\bm{\alpha}$ is obtained, the weighted sum of $\bm{f}_{subj}$ and $\bm{f}_{obj}$ can be computed as follows,
\begin{equation}
\label{eq2}
\bm{f}_{dual} = \bm{\alpha} \odot \bm{f}_{subj} + (1 - \bm{\alpha}) \odot \bm{f}_{obj},
\end{equation} 
 where \(\odot\) denotes the element-wise product and $\bm{f}_{dual}$ represents the weighted sum of $\bm{f}_{subj}$ and $\bm{f}_{obj}$.
\par
Finally, the vector $\bm{f}_{dual}$ is passed through a classifier, which consists of two linear layers with hidden dimensions of 1024, a ReLU activation function, and a dropout layer with a dropout probability of 0.15.
\paragraph{Implementation}
In an implementation, there are 50 training epochs, the batch size is set to 16, the optimizer is AdamW \citep{Loshchilov2017DecoupledWD} with a learning rate of 1e-6 and a weight decay rate of 0.01, the max length of input is set to 128, and the loss function is cross-entropy loss.
\par
Additionally, cross-validation is a data resampling method used to evaluate models and prevent overfitting. The basic form of cross-validation is k-fold cross-validation \citep{refaeilzadeh2009cross}. Therefore, the 5-fold cross-validation with a majority voting strategy is applied in the implementation and also proved to improve the performance of the proposed system. 
\par
All the experiments are conducted on a server with an Inter Xeon Gold 6142M CPU and an NVIDIA GeForce RTX 3090 GPU. 

